Zero-shot Triplet Extraction by Template Infilling

The task of triplet extraction aims to extract pairs of entities and their corresponding relations from unstructured text. Most existing methods train an extraction model on training data involving specific target relations, and are incapable of extracting new relations that were not observed at training time. Generalizing the model to unseen relations typically requires fine-tuning on synthetic training data which is often noisy and unreliable. We show that by reducing triplet extraction to a template infilling task over a pre-trained language model (LM), we can equip the extraction model with zero-shot learning capabilities and eliminate the need for additional training data. We propose a novel framework, ZETT (ZEro-shot Triplet extraction by Template infilling), that aligns the task objective to the pre-training objective of generative transformers to generalize to unseen relations. Experiments on FewRel and Wiki-ZSL datasets demonstrate that ZETT shows consistent and stable performance, outperforming previous state-of-the-art methods, even when using automatically generated templates. https://github.com/megagonlabs/zett/

==> backup.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
 \begin{tabular}{cl|c|cccc|cccc}
\hline
\multicolumn{3}{l}{\textbf{}} & \multicolumn{4}{c}{FewRel} & \multicolumn{4}{c}{Wiki-ZSL}  \\
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\# unseen\\ relations\end{tabular}} & \multicolumn{2}{l}{} & Single & \multicolumn{3}{c}{Multi} & Single & \multicolumn{3}{c}{Multi}  \\
& \multicolumn{1}{c}{Model} & \multicolumn{1}{c}{\# param} & \multicolumn{1}{c}{Acc} & P & R & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & P  & R  & F1  \\ \hline
\multirow{4}{*}{$m$=5} & TableSequence$\dagger$ & 240M & 11.82 & 15.23  & 1.91  & 3.40 & 14.47 & 43.68 & 3.51 & 6.29  \\
& Seq2seq w/ BART & 140M & 23.10 & 9.45 & \textbf{36.74} & 14.57 & 14.68 & 30.38 & \textbf{35.77} & 32.86 \\
& RelationPrompt & 264M & 24.36 & 30.70 & 25.36 & 32.74 & 15.70 & 32.49 & 35.07 & \textbf{33.73}  \\
& $\text{ZETT}_{\text{T5-small}}$ & 60M & 26.34 & 31.12 & 30.01 & 30.53 & 20.24 & 31.62 & 32.41 & 31.74 \\
& $\text{ZETT}_{\text{T5-base}}$ & 220M & \textbf{30.71} & \textbf{38.14} & 30.58 & \textbf{33.71} & \textbf{21.49} & \textbf{35.89} & 28.38 & 31.17  \\ \hline

\multirow{4}{*}{$m$=10}  & TableSequence$\dagger$ & 240M & 12.54 & 28.93  & 3.60  & 6.37 & 9.61 & \textbf{45.31} & 3.57 & 6.4  \\
& Seq2seq w/ BART & 140M & 16.51 & 6.40 & \textbf{41.70} & 11.02 & 10.09 & 18.64 & 22.37 & 20.33  \\
& RelationPrompt & 264M & 21.51 & 30.70 & 25.36 & 24.12 & 12.19 & 23.79 & 26.48  & 24.04  \\
& $\text{ZETT}_{\text{T5-small}}$ & 60M & 23.07 & 25.52 & 29.61 & 27.28 & 14.37 & 19.86 & \textbf{27.71} & 22.83 \\
& $\text{ZETT}_{\text{T5-base}}$ & 220M  & \textbf{27.79} & 30.65 & 32.44 & \textbf{31.28} & \textbf{17.16} & 24.49 & 26.99 & \textbf{24.87}  \\ \hline

\multirow{4}{*}{$m$=15}  & TableSequence$\dagger$ & 240M & 11.65  & 19.03  & 1.99  & 3.48 & 9.20 & \textbf{44.43} & 3.53 & 6.39  \\
& Seq2seq w/ BART & 140M & 11.91 & 4.61 & \textbf{36.39} & 8.15 & 7.24 & 12.23 & 14.40 & 13.23  \\
& RelationPrompt & 264M & 20.24 & \textbf{23.06} & 27.61 & 23.14 & 10.04 & 19.81 & 20.49  & 20.12 \\
& $\text{ZETT}_{\text{T5-small}}$ & 60M & 21.08 & 16.20 & 23.22 & 18.90 & 10.74 & 14.96 & 19.31 & 16.79 \\
& $\text{ZETT}_{\text{T5-base}}$ & 220M & \textbf{26.17} & 22.50 & 27.09 & \textbf{24.39} & \textbf{12.78} & 19.45 & \textbf{23.31} & \textbf{21.21} \\ \hline
\end{tabular}}
\caption{Accuracy (Acc) in the single-triplet, and Precision (P), Recall (R), and F1 score in the multi-triplet settings. $m$ denotes the number of unseen relations and the \# param column indicates the number of parameters of PLM used in each model. We experiment ZETT with T5-small ($\text{ZETT}_{\text{T5-small}}$) and T5-base ($\text{ZETT}_{\text{T5-base}}$). All reported results are averaged over five different data folds. Since we couldn't reproduce the results of RelationPrompt as same as reported in the paper, we report our results with three different random seeds. Results of $\dagger$ are taken from \citet{chia-etal-2022-relationprompt}}
\label{tab:main_results}
\end{table*}

\begin{table*}[ht]
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{ll}
\hline
\multicolumn{1}{c}{\textbf{Context}} & \multicolumn{1}{c}{\textbf{Template (Triplet)}} \\ \hline
\multirow{3}{90mm}{Spansion had its headquarters in Sunnyvale, California.} & \multirow{1}{90mm}{Spansion is headquartered in Sunnyvale, California} \\
& (Spansion, work location, Sunnyvale, California) \\
& (Spansion, location of formation, Sunnyvale) \\
\multirow{3}{90mm}{Born in Calcinate, the Province of Bergamo, Facchinetti started his career with hometown club Atalanta.} & \multirow{1}{90mm}{Province of Bergamo contains administrative territorial entity Calcinate} \\
& (Province of Bergamo, contains administrative territorial entity, Calcinate) \\
& \multirow{1}{90mm}{Facchinetti's job is club (Facchinetti, occupation, Atalanta)} \\
 \hline
\end{tabular}}
\caption{Error analysis}
\label{tab:error_analysis}
\end{table*}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
 \begin{tabular}{cl|cc|cc}
\hline
\multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{c}{FewRel} & \multicolumn{2}{c}{Wiki-ZSL}  \\
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\# unseen\\ relations\end{tabular}} & \multicolumn{1}{l}{} & Single & \multicolumn{1}{c}{Multi} & Single & \multicolumn{1}{c}{Multi}  \\
& \multicolumn{1}{c}{Model} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & F1  \\ \hline
\multirow{4}{*}{$m$=5} & TableSequence$\dagger$ & 11.82 & 3.40 & 14.47 & 6.29  \\
& Seq2seq & 23.10 & 14.57 & 14.68 & 32.86 \\
& RelationPrompt & 24.36 & 32.74 & 15.70 & \textbf{33.73}  \\
& $\text{ZETT}_{\text{small}}$ & 26.34 & 30.53 & 20.24 & 31.74 \\
& $\text{ZETT}_{\text{base}}$ & \textbf{30.71} & \textbf{33.71} & \textbf{21.49} & 31.72  \\ \hline

\multirow{4}{*}{$m$=10}  & TableSequence$\dagger$ & 12.09 & 6.37 & 9.61 & 6.4  \\
& Seq2seq & 16.67 & 11.02 & 9.94 & 20.33  \\
& RelationPrompt & 21.39 & 24.12 & 12.54 & 24.04  \\
& $\text{ZETT}_{\text{small}}$ & 23.12 & 27.28 & 14.37 & 22.83 \\
& $\text{ZETT}_{\text{base}}$ & \textbf{27.79} & \textbf{31.28} & \textbf{17.27} & \textbf{24.87}  \\ \hline

\multirow{4}{*}{$m$=15}  & TableSequence$\dagger$ & 11.65 & 3.48 & 9.20 & 6.39  \\
& Seq2seq & 11.91 & 8.15 & 7.24 & 13.23  \\
& RelationPrompt & 20.24 & 23.14 & 10.04 & 20.12 \\
& $\text{ZETT}_{\text{small}}$ & 21.08 & 18.90 & 10.74 & 16.79 \\
& $\text{ZETT}_{\text{base}}$ & \textbf{26.17} & \textbf{24.39} & \textbf{12.78} & \textbf{21.21} \\ \hline
\end{tabular}}
\caption{Accuracy (Acc) in the single-triplet and F1 score in the multi-triplet settings. $m$ denotes the number of unseen relations. We experiment ZETT with T5-small ($\text{ZETT}_{\text{small}}$) and T5-base ($\text{ZETT}_{\text{base}}$). All reported results are averaged over five different data folds. Results of $\dagger$ are taken from \citet{chia-etal-2022-relationprompt}.}
\label{tab:main_results}
\end{table}

\subsection{Human Evaluation}
\label{sec:human_eval}
The datasets we used in experiments are mainly made by distant supervision \citep{sorokin-gurevych-2017-context}.
The main strategy of distant supervision is automatically collecting sentences mentioning head and tail entities, given a factual triplet.
However, we observe many examples where the context is not related to the given relation or the triplet cannot be inferred from the context.
For example, the context ``This lizard lives in the southwestern part of Africa, in Namibia and South Africa.'' is annotated with the triple (South Africa, \textit{shares border with}, Namibia). Although this triplet is true, it does not follow from the given text context. Another type of error is a false negative. We find that some of ZETT's predictions are counted false, although they are actually true. To give an example, for the context ``Google released Android 7.1.1 Nougat for the Pixel C in December 2016.'', the labeled answer is (Pixel C, \textit{operating system}, Android). However, our model predicts (Pixel C, \textit{owned by}, Google), and this is also true.

Based on the these observations, we conducted a human evaluation to obtain more precise results. We manually annotated 1,000 examples, top 5 results for 200 contexts. The contexts are randomly sampled from the single-triplet test set of $m$=10 on the Wiki-ZSL. Annotators are guided to assess top 5 predictions of $\text{ZETT}_{\text{base}}$.
Three PhDs knowledgeable in this domain participated in the evaluation, and the annotation results in substantial agreement with a Kappa coefficient of 0.75. We regard the true triplets when two annotators agree that the instance is true. As a result of human evaluation, we found 127 incorrectly labeled triplets in the original dataset, and discovered 50 more true triplets which were labeled as false. When we re-evaluate $\text{ZETT}_{\text{base}}$ with this manually annotated set, the observed accuracy increases from 18.0 to 30.2. This human annotated test set will be released.

\subsection{ZETT for Entity Extraction}
Since most relations are not symmetric, i.e., ($h$, $r$, $t$) $\neq$ ($t$, $r$, $h$), identifying which entity should be head or tail is also critical in triplet extraction. One of the benefits of using a template in ZETT is that a template provides implicit entity type constraints through natural language sentences, which helps identifying head and tail entities correctly. In this section, we evaluate the effectiveness of ZETT on the entity extraction task which aims to predict head and tail entities given an input sentence and a relation. ZETT can be used for entity extraction without changing the model or input format by providing the gold relation's template for the input. Experimental settings are the same as in zero-shot triplet extraction, where we fine-tune the model with training examples of seen relations and test on examples which relations are unseen. For the metric, we use the accuracy with each gold entity and model's prediction.

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lccc|ccc}
\hline
 & \multicolumn{3}{c}{FewRel} & \multicolumn{3}{c}{Wiki-ZSL} \\
\multicolumn{1}{c}{Model} & $m$=5  & $m$=10 & \multicolumn{1}{c}{$m$=15} & $m$=5  & $m$=10 & \multicolumn{1}{c}{$m$=15} \\ \hline
Seq2seq & 38.6 & 42.5	& 38.6	& 36.2 & 35.6	& 33.9 \\
RelationPrompt & 35.8 & 36.7 & 36.8 & 33.0 & 32.0 & 29.6 \\
$\text{ZETT}_{\text{T5-small}}$ & 40.1 & 43.0 & 43.8 & 35.0 & 33.0 & 29.9 \\
$\text{ZETT}_{\text{T5-base}}$ & \textbf{46.7} & \textbf{50.2} & \textbf{50.5} & \textbf{36.2} & \textbf{37.1} & \textbf{34.1} \\ \hline
\end{tabular}}
\caption{Results of entity extraction (Accuracy). We evaluate whether the model exactly predicts head and tail entities.}
\label{tab:entity_extraction}
\end{table}

\paragraph{Results}
Table \ref{tab:entity_extraction} shows the results of entity extraction. Since the RelationPrompt relies on synthetic data, which are noisy and not correctly labeled, the performance drops when the model is fine-tuned on synthetic data. Another issue of the RelationPrompt is the formatted text used for triplet generation, such as "Head Entity: <head>, Tail Entity : <tail>, Relation : <relation>". This is easy to fail to identify head and tail entities since there is no information that the target entity is subjective or objective.
On the other hand, ZETT shows consistent improvements over the previous models. ZETT can benefit from natural language templates which provide the implicit constraints of entity types. For example, for the relation \textit{participant in}, the template ``<head> is a participant in <tail>'' gives implicit type constraints such that the <head> should be a subject of the relation \textit{participant in}, such as human or sports team, and the <tail> should be an object of that the subject can be \textit{participant in}, such as contest or sports game. This information helps the model to correctly predict the head and tail entities.

\subsubsection{Choice of templates}
Templates provide the benefits of leveraging PLMs as in the form of a natural language sentence. However, making hand-crafted templates requires human labor and using a single template for each relation might not be an optimal solution \citep{gao-etal-2021-making,sanh2022multitask}. Several studies have introduced methods to automatically generate templates. In this section, we investigate how ZETT works with three different automated templates: mining-based \citep{jiang-etal-2020-know}, paraphrasing-based \citep{jiang-etal-2020-know}, and automating prompt generation \citep{gao-etal-2021-making}.

\paragraph{Methods for automated templates}

\textbf{1) Mining-based:}
Mining-based generation is based on the distant supervision over Wikipedia articles. 
After collecting sentences mentioning both head and tail entities, they use the middle-word rule, which regards middle words between two entities as an indication of the relation, and dependency parsing which obtains the template by mining the phrase span between entity nodes in the tree.

\textbf{2) Paraphrasing-based:}
This approach expands the original templates by paraphrasing them to improve lexical diversity. 
They paraphrase the highest-ranked mined templates for each relation.
For the paraphrasing technique, they use back-translation with the model trained on English-German machine translation.

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{} & Single  & \multicolumn{3}{c}{Multi}        \\ 
\multicolumn{1}{c}{Model} & Acc  & P & R  & F1        \\ \hline
Seq2seq & 8.09 & 9.88 & 11.55 & 10.64  \\
RelationPrompt & 11.47 & 16.87 & 17.21 & 16.88 \\ \hline
$\text{ZETT}_{\text{small}}$ w/ \textit{Manual} & 14.31 & 15.46 & 17.85 & 16.34 \\
$\text{ZETT}_{\text{small}}$ w/ \textit{Mining}   & 13.34	& 12.21 & {28.51} & 16.95 \\
$\text{ZETT}_{\text{small}}$ w/ \textit{Paraphrase}      & 11.36	& 12.31	& 28.31	& 16.99 \\ 
$\text{ZETT}_{\text{small}}$ w/ \textit{Auto-gen} & 12.18 & 12.58 & 22.89 & 16.14 \\ \hline
$\text{ZETT}_{\text{base}}$ w/ \textit{Manual} & \textbf{17.60} & \textbf{25.12} & 15.81 & 19.25 \\
$\text{ZETT}_{\text{base}}$ w/ \textit{Mining}   & 15.73	& 21.21 & 30.19 & 24.77 \\  
$\text{ZETT}_{\text{base}}$ w/ \textit{Paraphrase} & 15.10 &	22.04 & \textbf{31.22} & \textbf{25.60} \\ 
$\text{ZETT}_{\text{base}}$ w/ \textit{Auto-gen} & 12.94 & 17.43 & 18.47 & 17.31 \\
\hline
\end{tabular}}
\caption{Results with automatically generated templates for unseen relations, in the single- and multi-triplet settings. \textit{Manual} refers to templates manually created by us.}
\label{tab:auto_template}
\end{table}

\textbf{3) Automating prompt generation:}
\citet{gao-etal-2021-making} proposed the template generation method as a prediction of the masked span \texttt{<X>} between head and tail entities. The key idea of this approach is generating templates using a few labeled examples and searching the most generalized templates.
Given a set of labeled examples $\mathcal{D}_l$, template generation can be formulated as follows:
\begin{quote}
\small
\texttt{[context]}. \texttt{[H]} \texttt{<X>} \texttt{[T]} $\rightarrow$ template \\ 
\texttt{[context]}. \texttt{[T]} \texttt{<X>} \texttt{[H]} $\rightarrow$ template
\end{quote}
We generate multiple templates for each example with a large beam size (e.g., 20).
Then we score all templates with the LM probability 
with the T5-base model on $\mathcal{D}_l$. 
Lastly, we pick the top-$k$ templates with the highest score.

This method is originally designed for few-shot learning which assumes that there are $n$ labeled examples for each class. Following \citet{gao-etal-2021-making}, we use $n$=32 labeled examples for each relation in our experiments. However, we note that these are not used for fine-tuning the model, but only for generating templates automatically.

\paragraph{Experimental settings}
For experiments with mining and paraphrase-based templates, we used the templates provided by LPAQA \citep{jiang-etal-2020-know}. However, not all templates are provided for FewRel and Wiki-ZSL datasets.  Therefore, we use a subset of the relations in Wiki-ZSL which overlaps with LPAQA. As a result, the total number of relations is 36, which we split into 26/5/5 for train/dev/test sets. As in our main experiments, we use five data folds with different random seeds and report the average of five data folds. Statistics for each fold are provided in the Appendix (Table \ref{tab:auto_stat}).
Since automated methods provide multiple templates for each relation, we experimented with $k \in \{1, 2, 3, 4, 5\}$ templates and found $k$=2 to perform the best.

\paragraph{Results with Automated Templates}
Table \ref{tab:auto_template} shows the results of ZETT with automated templates. We compare the results with automated templates and the results with manual templates in Table \ref{tab:man_template}. In experiments with the $\text{ZETT}_{\text{small}}$ model, we obtained an accuracy of 13.34\% with the mining-based templates in the single-triplet setting. This is less than 1\% point difference with the manual template's result, and we find that this gap can be overcome with a larger T5 model, $\text{ZETT}_{\text{base}}$. In the multi-triplet setting, both the mining and paraphrasing-based performs better than manual templates, particularly improving the recalls. Although the automatically generated templates are noisy and less accurate, we can obtain more diverse templates. We can conclude that automated templates can be incorporated into $\text{ZETT}$, and multiple templates can help the model generalize better to unseen relations.

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lccc|ccc}
\hline
 & \multicolumn{3}{c}{FewRel} & \multicolumn{3}{c}{Wiki-ZSL} \\
\multicolumn{1}{c}{Model} & $m$=5  & $m$=10 & \multicolumn{1}{c}{$m$=15} & $m$=5  & $m$=10 & \multicolumn{1}{c}{$m$=15} \\ \hline
Seq2seq & 38.6 & 42.5	& 38.6	& 36.2 & 35.6	& 33.9 \\
RelationPrompt & 35.8 & 36.7 & 36.8 & 33.0 & 32.0 & 29.6 \\
$\text{ZETT}_{\text{small}}$ & 40.1 & 43.0 & 43.8 & 35.0 & 33.0 & 29.9 \\
$\text{ZETT}_{\text{base}}$ & \textbf{46.7} & \textbf{50.2} & \textbf{50.5} & \textbf{36.2} & \textbf{37.1} & \textbf{34.1} \\ \hline
\end{tabular}}
\caption{Results of entity extraction (Accuracy). We evaluate whether the model exactly predicts head and tail entities.}
\label{tab:entity_extraction}
\end{table}

\subsubsection{Entity Extraction and Relation Classification}
Triplet extraction can be conducted by combining two sub-tasks: entity extraction and relation classification. In this section, we analyze ZETT's performance on each task.
For entity extraction, ZETT can be applied without changing the model or input format by providing the gold relation's template for the input. Since most relations are not symmetric, i.e., ($h$, $r$, $t$) $\neq$ ($t$, $r$, $h$), identifying which entity should be head or tail is also critical in triplet extraction. Table \ref{tab:entity_extraction} shows the results of entity extraction. Since the RelationPrompt relies on synthetic data, which are noisy and not correctly labeled, the performance drops when the model is fine-tuned on synthetic data. Another issue of the RelationPrompt is the formatted text used for triplet generation, such as "Head Entity: <head>, Tail Entity : <tail>, Relation : <relation>". This is easy to fail to identify head and tail entities since there is no information that the target entity is subjective or objective. On the other hand, ZETT shows consistent improvements over the previous models. ZETT can benefit from natural language templates which provide the implicit constraints of entity types. For example, for the relation \textit{participant in}, the template ``<head> is a participant in <tail>'' gives implicit type constraints such that the <head> should be a subject of the relation \textit{participant in}, such as human or sports team, and the <tail> should be an object of that the subject can be \textit{participant in}, such as contest or sports game. This information helps the model to correctly predict the head and tail entities.

\begin{table}[h]
    \centering
    \small
    \begin{tabular}{c|c|c|c}
    \hline
         random seed & \# train & \# valid & \# test \\ \hline
         0 & 28,474 & 5,132 & 6,225 \\
         1 & 25,094 & 7,834 & 7,004 \\
         2 & 25,509 & 5,642 & 8,790 \\
         3 & 25,971 & 7,051 & 6,885 \\
         4 & 28,974 & 6,195 & 4,706 \\\hline
    \end{tabular}
    \caption{The number of examples in each data fold in experiments for automated templates.}
    \label{tab:auto_stat}
\end{table}

==> supplementary_materials.tex <==
\section{List of All Templates}
\begin{center}
\begin{small}
\begin{longtable}[ht]{p{1in}|p{0.4in}|p{1.8in}|p{2.5in}}
\hline
\multicolumn{1}{c}{\textbf{Relation}} & \multicolumn{1}{c}{\textbf{Id}} & \multicolumn{1}{c}{\textbf{Template}} & \multicolumn{1}{c}{\textbf{Description}} \\ \hline
applies to jurisdiction & P1001 & \texttt{[H]} is a legal term in \texttt{[T]} . & the item (institution, law, public office, public register...) or statement belongs to or has power over or applies to the value (a territorial jurisdiction: a country, state, municipality, ...) \\
field of work & P101 & \texttt{[H]} works in the field of \texttt{[T]} . & specialization of a person or organization \\
member of political party & P102 & \texttt{[H]} is a member of political party \texttt{[T]} . & the political party of which a person is or has been a member or otherwise affiliated \\
taxon rank & P105 & \texttt{[H]} is a taxon rank of \texttt{[T]} . & level in a taxonomic hierarchy \\
occupation & P106 & \texttt{[H]}'s job is \texttt{[T]} . & occupation of a person \\
league & P118 & \texttt{[T]} is a league of \texttt{[H]} . & league in which team or player plays or has played in \\
publisher & P123 & \texttt{[H]} is published by \texttt{[T]} . & organization or person responsible for publishing books, periodicals, printed music, podcasts, games or software \\
owned by & P127 & \texttt{[H]} is owned by \texttt{[T]} . & owner of the subject \\
instrument & P1303 & \texttt{[H]} plays \texttt{[T]} . & musical instrument that a person plays or teaches or used in a music occupation \\
located in the administrative territorial entity & P131 & \texttt{[H]} is located in the administrative territorial entity of \texttt{[T]} . & the item is located on the territory of the following administrative entity. \\
participant in & P1344 & \texttt{[H]} is a participant in \texttt{[T]} . & event in which a person or organization was/is a participant \\
winner & P1346 & \texttt{[T]} is a winner of \texttt{[H]} . & winner of a competition or similar event, not to be used for awards \\
movement & P135 & \texttt{[H]} is part of movement \texttt{[T]} . & literary, artistic, scientific or philosophical movement or scene associated with this person or work \\
genre & P136 & \texttt{[T]} is a genre of \texttt{[H]} . & creative work's genre or an artist's field of work \\
operator & P137 & \texttt{[T]} is an operator of \texttt{[H]} . & person, profession, or organization that operates the equipment, facility, or service \\
religion & P140 & \texttt{[H]}'s religion is \texttt{[T]}. & religion of a person, organization or religious building, or associated with this subject \\
licensed to broadcast to & P1408 & \texttt{[H]} is lisensed to broadcast to \texttt{[T]} . & place that a radio/TV station is licensed/required to broadcast to \\
nominated for & P1411 & \texttt{[H]} is nominated for \texttt{[T]} . & award nomination received by a person, organisation or creative work \\
heritage designation & P1435 & \texttt{[H]} is designated as heritage by \texttt{[T]} . & heritage designation of a cultural or natural site \\
contains administrative territorial entity & P150 & \texttt{[H]} contains administrative territorial entity \texttt{[T]} . & direct subdivisions of an administrative territorial entity \\
follows & P155 & \texttt{[H]} follows \texttt{[T]} . & immediately prior item in a series of which the subject is a part \\
followed by & P156 & \texttt{[H]} is followed by \texttt{[T]} . & immediately following item in a series of which the subject is a part \\
headquarters location & P159 & \texttt{[H]} is headquartered in \texttt{[T]} . & city, where an organization's headquarters is or has been situated \\
performer & P175 & \texttt{[T]} is a performer of \texttt{[H]} . & actor, musician, band or other performer associated with this role or musical work \\
manufacturer & P176 & \texttt{[H]} is manufactured by \texttt{[T]} . & manufacturer or producer of this product \\
crosses & P177 & \texttt{[H]} crosses \texttt{[T]} . & obstacle (body of water, road, railway...) which this bridge crosses over or this tunnel goes under \\
developer & P178 & \texttt{[H]} is developed by \texttt{[T]} . & organization or person that developed the item \\
after a work by & P1877 & \texttt{[H]} after a work by \texttt{[T]} . & artist whose work strongly inspired/ was copied in this item \\
participating team & P1923 & \texttt{[T]} is a participating team in \texttt{[H]} . & like Participant but for teams \\
located in or next to body of water & P206 & \texttt{[H]} is located in or next to body of water \texttt{[T]} . & body of water on or next to which a place is located \\
competition class & P2094 & \texttt{[H]} is in the competition class \texttt{[T]} . & official classification by a regulating body under which the subject (events, teams, participants, or equipment) qualifies for inclusion \\
father & P22 & \texttt{[T]} is a father of \texttt{[H]} . & male parent of the subject \\
military branch & P241 & \texttt{[H]} is a military branch of \texttt{[T]} . & branch to which this military unit, award, office, or person belongs \\
mother & P25 & \texttt{[T]} is a mother of \texttt{[H]} . & female parent of the subject \\
spouse & P26 & \texttt{[H]} is a spouse of \texttt{[T]} . & the subject has the object as their spouse \\
record label & P264 & \texttt{[H]} is represented by the record label \texttt{[T]} . & brand and trademark associated with the marketing of subject music recordings and music videos \\
country of citizenship & P27 & \texttt{[H]} is citizen of \texttt{[T]} . & the object is a country that recognizes the subject as its citizen \\
location & P276 & \texttt{[H]} is located in \texttt{[T]} . & location of the object, structure or event. \\
operating system & P306 & \texttt{[H]}'s operating system is \texttt{[T]} . & operating system (OS) on which a software works or the OS installed on hardware \\
sibling & P3373 & \texttt{[H]} is a sibling of \texttt{[T]} . & the subject and the object have the same parents (brother, sister, etc.) \\
sports season of league or competition & P3450 & \texttt{[H]} is a sports season of league or competition of \texttt{[T]} . & property that shows the competition of which the item is a season \\
subsidiary & P355 & \texttt{[T]} is a subsidiary of \texttt{[H]} . & subsidiary of a company or organization \\
part of & P361 & \texttt{[H]} is part of \texttt{[T]} . & object of which the subject is a part \\
original language of film or TV show & P364 & \texttt{[H]} is the original language of \texttt{[T]}. & language in which a film or a performance work was originally created \\
position held & P39 & \texttt{[H]} holds a position \texttt{[T]} . & subject currently or formerly holds the object position or public office \\
child & P40 & \texttt{[T]} is a child of \texttt{[H]} . & subject has object as child \\
platform & P400 & \texttt{[T]} is a platform of \texttt{[H]} . & platform for which a work was developed or released, or the specific platform version of a software product \\
mouth of the watercourse & P403 & \texttt{[T]} is a mouth of the watercourse of \texttt{[H]} . & the body of water to which the watercourse drains \\
language of work or name & P407 & \texttt{[H]} is written in \texttt{[T]} . & language associated with this creative work (such as books, shows, songs, broadcasts or websites) or a name \\
military rank & P410 & \texttt{[H]}'s military rank is \texttt{[T]} . & military rank achieved by a person, or military rank associated with a position \\
voice type & P412 & \texttt{[H]}'s voice type is \texttt{[T]} . & person's voice type. expected values: soprano, mezzo-soprano, contralto, countertenor, tenor, baritone, bass (and derivatives) \\
position played on team / speciality & P413 & \texttt{[H]} plays the position \texttt{[T]} . & position or specialism of a player on a team \\
original broadcaster & P449 & \texttt{[T]} is the original broadcaster of \texttt{[H]} . & network or service that originally broadcast a radio or television program \\
mountain range & P4552 & \texttt{[T]} is a moutain range of \texttt{[H]} . & range or subrange to which the geographical item belongs \\
said to be the same as & P460 & \texttt{[H]} is said to be the same as \texttt{[T]} . & this item is said to be the same as that item \\
member of & P463 & \texttt{[H]} is a member of \texttt{[T]} . & organization, club or musical group to which the subject belongs. \\
occupant & P466 & \texttt{[T]} is an occupant of \texttt{[H]} . & person or organization occupying property \\
country of origin & P495 & \texttt{[H]} was created in the country \texttt{[T]} . & country of origin of this item (creative work, food, phrase, product, etc.) \\
has part & P527 & \texttt{[H]} has part of \texttt{[T]} . & part of this subject \\
residence & P551 & \texttt{[H]} lives in \texttt{[T]} . & the place where the person is or has been, resident \\
director & P57 & \texttt{[T]} is a director of \texttt{[H]} . & director(s) of film, TV-series, stageplay, video game or similar \\
screenwriter & P58 & \texttt{[T]} wrote the script for \texttt{[H]} . & person(s) who wrote the script for subject item \\
constellation & P59 & \texttt{[H]} is in the constellation \texttt{[T]} . & the area of the celestial sphere of which the subject is a part \\
head of government & P6 & \texttt{[T]} is the head of goverment of \texttt{[H]} . & head of the executive power of this town, city, municipality, state, country, or other governmental body \\
sport & P641 & \texttt{[H]} plays a sport \texttt{[T]} . & sport that the subject participates or participated in or is associated with \\
characters & P674 & \texttt{[T]} is a character of \texttt{[H]} . & characters which appear in this item (like plays, operas, operettas, books, comics, films, TV series, video games) \\
located on terrain feature & P706 & \texttt{[H]} is located on terrain feature \texttt{[T]} . & located on the specified (geo)physical feature. \\
participant & P710 & \texttt{[T]} is a participant in \texttt{[H]} . & person, group of people or organization (object) that actively takes/took part in an event or process (subject) \\
location of formation & P740 & \texttt{[H]} was established in \texttt{[T]} . & location where a group or organization was formed \\
distributed by & P750 & \texttt{[H]} is distributed by \texttt{[T]} . & distributor of a creative work; distributor for a record label; news agency; film distributor \\
notable work & P800 & \texttt{[T]} is notable work of \texttt{[H]} . & notable scientific, artistic or literary work, or other work of significance among subject's works \\
architect & P84 & \texttt{[T]} is an architect of \texttt{[H]} . & person or architectural firm responsible for designing this building \\
composer & P86 & \texttt{[T]} is a composer of \texttt{[H]} . & person(s) who wrote the music \\
main subject & P921 & \texttt{[T]} is the main subject of \texttt{[H]}. & primary topic of a work \\
place served by transport hub & P931 & \texttt{[T]} is a place served by transport hub \texttt{[H]} . & territorial entity or entities served by this transport hub (airport, train station, etc.) \\
work location & P937 & \texttt{[H]} worked in \texttt{[T]} . & location where persons or organisations were actively participating in employment, business or other work \\
tributary & P974 & \texttt{[T]} is a tributary of \texttt{[H]} . & watercourse that flows into an other one \\
successful candidate & P991 & \texttt{[T]} is a successful candidate of \texttt{[H]} . & person(s) elected after the election \\
country & P17 & \texttt{[T]} is a country of \texttt{[H]} . & sovereign state of this item (not to be used for human beings) \\
instance of & P31 & \texttt{[H]} is a \texttt{[T]} . & that class of which this subject is a particular example and member \\
inception & P571 & \texttt{[T]} is created in \texttt{[H]} . & time when an entity begins to exist \\
subclass of & P279 & \texttt{[H]} is a subclass of \texttt{[T]} . & this item is a subclass (subset) of that item \\
capital & P36 & \texttt{[T]} is a capital of \texttt{[H]} . & seat of government of a country, province, state or other type of administrative territorial entity \\
is a list of & P360 & \texttt{[H]} is a list of \texttt{[T]} . & common element between all listed items \\
place of death & P20 & \texttt{[H]} died in \texttt{[T]} . & most specific known (e.g. city instead of country, or hospital instead of city) death location of a person, animal or fictional character \\
place of birth & P19 & \texttt{[H]} was born in \texttt{[T]} . & most specific known (e.g. city instead of country, or hospital instead of city) birth location of a person, animal or fictional character \\
continent & P30 & \texttt{[T]} is the continent of \texttt{[H]} . & continent of which the subject is a part \\
educated at & P69 & \texttt{[H]} studied at \texttt{[T]} . & educational institution attended by subject \\
author & P50 & \texttt{[H]} is written by \texttt{[T]} . & main creator(s) of a written work (use on works, not humans) \\
conflict & P607 & \texttt{[H]} is participated in the battle \texttt{[T]} . & battles, wars or other military engagements in which the person or item participated \\
official language & P37 & \texttt{[T]} is an official language in \texttt{[H]} . & language designated as official by this item \\
facet of & P1269 & \texttt{[H]} is one facet of \texttt{[T]} . & topic of which this item is an aspect, item that offers a broader perspective on the same topic \\
award received & P166 & \texttt{[H]} received an award \texttt{[T]} . & award or recognition received by a person, organization or creative work \\
date of birth & P569 & \texttt{[T]} was born in \texttt{[H]} . & date on which the subject was born \\
influenced by & P737 & \texttt{[H]} is influenced by \texttt{[T]} . & this person, idea, etc. is informed by that other person, idea, etc. \\
employer & P108 & \texttt{[H]} worked for \texttt{[T]} . & person or organization for which the subject works or worked \\
date of death & P570 & \texttt{[T]} died in \texttt{[H]} & date on which the subject died \\
diplomatic relation & P530 & \texttt{[H]} and \texttt{[T]} have diplomatic relations . & diplomatic relations of the country \\
student & P802 & \texttt{[T]} is a student of \texttt{[H]} . & notable student(s) of the subject individual \\
founded by & P112 & \texttt{[H]} is founded by \texttt{[T]} . & founder or co-founder of this organization, religion or place \\
field of this occupation & P425 & \texttt{[T]} is a field of \texttt{[H]} . & field corresponding to this occupation or profession \\
creator & P170 & \texttt{[H]} is created by \texttt{[T]} . & maker of this creative work or other object \\
product or material produced & P1056 & \texttt{[H]} products \texttt{[T]} . & material or product produced by a government agency, business, industry, facility, or process \\
industry & P452 & \texttt{[H]} is in the \texttt{[T]} industry . & specific industry of company or organization \\
family & P53 & \texttt{[H]} is a family of \texttt{[T]} . & family, including dynasty and nobility houses \\
item operated & P121 & \texttt{[H]} operates \texttt{[T]} . & equipment, installation or service operated by the subject \\
named after & P138 & \texttt{[H]} is named after \texttt{[T]} . & entity or event that inspired the subject's name, or namesake \\
given name & P735 & \texttt{[T]} is first name of \texttt{[H]} . & first name or another given name of this person \\
producer & P162 & \texttt{[H]} is produced by \texttt{[T]} . & person(s) who produced the film, musical work, theatrical production, etc. \\
publication date & P577 & \texttt{[T]} is first published in \texttt{[H]} . & date or point in time when a work was first published or released \\
narrative location & P840 & \texttt{[H]} takes place in \texttt{[T]} . & the narrative of the work is set in this location \\
production company & P272 & \texttt{[H]} is produced by studio \texttt{[T]} . & company that produced this film, audio or performing arts work \\
languages spoken, written or signed & P1412 & \texttt{[H]} uses language \texttt{[T]} . & language(s) that a person or a people speaks, writes or signs, including the native language(s) \\
family name & P734 & \texttt{[H]}'s last name is \texttt{[T]} . & part of full name of person \\
organization directed by the office or position & P2389 & \texttt{[H]} is a head of \texttt{[T]} . & organization which is directed by this office \\
connecting line & P81 & \texttt{[H]} is connected to \texttt{[T]} . & railway line(s) subject is directly connected to \\
member of sports team & P54 & \texttt{[H]} is a member of \texttt{[T]} team . & sports teams or clubs that the subject represents or represented \\
part of the series & P179 & \texttt{[H]} is a part of the series \texttt{[T]} . & series which contains the subject \\
parent astronomical body & P397 & \texttt{[H]} is an orbit of \texttt{[T]} . & major astronomical body the item belongs to \\
lyrics by & P676 & \texttt{[T]} wrote the lyrics of \texttt{[H]} . & author of song lyrics \\
different from & P1889 & \texttt{[H]} is different from \texttt{[T]} . & item that is different from another item, with which it may be confused \\
replaces & P1365 & \texttt{[H]} succeeds \texttt{[T]} . & person, state or item replaced \\
sports discipline competed in & P2416 & \texttt{[H]} competed in a \texttt{[T]} sport . & discipline an athlete competed in within a sport \\
drafted by & P647 & \texttt{[H]} was drafted by \texttt{[T]} . & which team the player was drafted by \\
based on & P144 & \texttt{[H]} is based on \texttt{[T]} . & the work(s) used as the basis for subject item \\
opposite of & P461 & \texttt{[H]} is opposite of \texttt{[T]} . & item that is the opposite of this item \\
lowest point & P1589 & \texttt{[H]} is the lowest point of \texttt{[T]} . & point with lowest elevation in the country, region, city or area \\
has quality & P1552 & \texttt{[H]} has characteristic \texttt{[T]} . & the entity has an inherent or distinguishing non-material characteristic \\
use & P366 & \texttt{[H]} is used in \texttt{[T]} . & main use of the subject (includes current and former usage) \\
from narrative universe & P1080 & \texttt{[H]} is featured in universe \texttt{[T]} . & subject's fictional entity is in the object narrative \\
made from material & P186 & \texttt{[H]} is made from \texttt{[T]} . & material the subject or the object is made of or derived from \\
shares border with & P47 & \texttt{[T]} shares border with \texttt{[H]} . & countries or administrative subdivisions, of equal level, that this item borders, either by land or water \\
twinned administrative body & P190 & \texttt{[H]} and \texttt{[T]} are twin cities . & twin towns, sister cities, twinned municipalities and other localities that have a partnership or cooperative agreement, either legally or informally acknowledged by their governments \\
cast member & P161 & \texttt{[T]} is an actor in \texttt{[H]} . & actor in the subject production \\
located on astronomical body & P376 & \texttt{[H]} is on the planet \texttt{[T]} . & astronomical body on which features or places are situated \\ \hline
\caption{Manually built templates used in experiments.}
\label{tab:man_template}
\end{longtable}
\end{small}
\end{center}
